Randomized Smoothing under Attack: How Good is it in Pratice?

Randomized smoothing is a recent and celebrated solution to certify the robustness of any classifier. While it indeed provides a theoretical robustness against adversarial attacks, the dimensionality of current classifiers necessarily imposes Monte Carlo approaches for its application in practice. This paper questions the effectiveness of randomized smoothing as a defense, against state of the art black-box attacks. This is a novel perspective, as previous research works considered the certification as an unquestionable guarantee. We first formally highlight the mismatch between a theoretical certification and the practice of attacks on classifiers. We then perform attacks on randomized smoothing as a defense. Our main observation is that there is a major mismatch in the settings of the RS for obtaining high certified robustness or when defeating black box attacks while preserving the classifier accuracy.

==> 6_annexex.tex <==
% !TEX root =  fastbbearl.tex
\section{Full Results}
\label{sec:black_box_attack}

\begin{table}[ht]
	\begin{center}
		\begin{tabular}{|c|c|c|c|c|c|}
			\hline
			Model & Attack & Noise & Monte Carlo & $D_{1/2}$ & Mean Distance\\
			\hline
			\multirow{12}{*}{ResNet50} & \multirow{4}{*}{SurFree} & \multicolumn{2}{|c|}{Base} & 6.93 & 5.21 \\
			& & 0.06 & 10 & 38.42 & 55.11 \\
			& & 0.06 & 50 & & \\
			& & 0.06 & 200 & & \\
			& \multirow{4}{*}{RayS} & \multicolumn{2}{|c|}{Base} & & \\
			& & 0.06 & 10 & & \\
			& & 0.06 & 50 & & \\
			& & 0.06 & 200 & & \\
			& \multirow{4}{*}{HopSkipJump} & \multicolumn{2}{|c|}{Base} & & \\
			& & 0.06 & 10 & & \\
			& & 0.06 & 50 & & \\
			& & 0.06 & 200 & & \\
			\hline
			\multirow{12}{*}{ResNet50 Retrained} & \multirow{4}{*}{SurFree} & & & & \\
			& \multirow{4}{*}{RayS} & & & & \\
			& \multirow{4}{*}{HopSkipJump} & & & & \\
			
			\hline
		\end{tabular}
	\end{center}
	\caption{Results for Resnet50. Noise selected to have negligible on the accuracy.}
	\label{tab:multicol}
\end{table}



